LiteVGGT: Boosting Vanilla VGGT via Geometry-aware Cached Token Merging

3D vision foundation models like Visual Geometry Grounded Transformer (VGGT) have advanced greatly in geometric perception. However, it is time-consuming and memory-intensive for long sequences, limiting application to large-scale scenes beyond hundreds of images. To address this, we propose LiteVGGT, achieving up to 10x speedup and substantial memory reduction, enabling efficient processing of 1000-image scenes. We derive two key insights for 3D reconstruction: (1) tokens from local image regions have inherent geometric correlations, leading to high similarity and computational redundancy; (2) token similarity across adjacent network layers remains stable, allowing for reusable merge decisions. Guided by these, we design a simple yet efficient strategy, dubbed geometry-aware cached token merging. We analyze each token's geometric importance, optimizing anchor token selection to better preserve key information for reconstruction. We also cache and reuse merge indices across layers, substantially reducing latency with minimal accuracy impact. This strategy retains VGGT's core performance, enabling efficient fine-tuning and FP8 quantization for further gains. Extensive experiments validate LiteVGGT's effectiveness, scalability, and robustness. Project page: https://garlicba.github.io/LiteVGGT/

==> sec/3_method_old.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.8\linewidth,height=5cm]{sec/figures/global_time.pdf}
  \caption{Latency analysis of the VGGT components. As the number of images increases, Global Attention gradually dominates the inference time.}
  \label{fig:global_time}
\end{figure}

\section{Method}
We introduce LiteVGGT, a lightweight version of VGGT that achieves a 10× speedup while maintaining high accuracy. We begin by first revisiting the architecture of VGGT in Sec. 3.1, followed by our bottleneck analysis in Sec. 3.2. In Sec. 3.3, we describe our gs-driven and cached token merge strategy, and finally, in Sec. 3.4, we present our fine-tuning and FP8 quantization for further optimization.

\subsection{VGGT Architecture and Bottleneck Analysis}

Visual Geometry Grounded Transformer (VGGT) \cite{Wang2025a} is a recent architecture designed to predict all key 3D attributes from image sequences of arbitrary length. For any input sequence \( \mathcal{I} = \{I_i\}_{i=1}^N \) of \( N \) RGB frames, VGGT first tokenizes each frame using a pretrained vision backbone \( \mathcal{F}(\cdot) \), such as DINOv2, producing

\begin{equation}
\mathbf{X} = \{x_i \mid x_i = \mathcal{F}(I_i)\}_{i=1}^N, \quad x_i \in \mathbb{R}^{n \times d}
\tag{1}
\end{equation}

where \( n \) denotes the token length after patching and \( d \) is the feature dimension.

To enable multi-attribute reasoning, VGGT augments each frame with one \textit{camera token} and four \textit{register tokens}, which are responsible for aggregating different 3D attributes (e.g., camera parameters, scene geometry). Notably, VGGT introduces two distinct sets of these special tokens: one set \( t_f \in \mathbb{R}^{5 \times d} \) is reserved for the first frame, defining the coordinate system of its camera as the world coordinate system, while another set \( t_0 \in \mathbb{R}^{5 \times d} \) is shared by all subsequent frames. 

% Holistic spatial-temporal relationships for consistency
% Enhance local understanding
% Capture local details
The special tokens are concatenated with their corresponding patch tokens and fed into the 24-layer frame-global attention. The output tokens are then passed to separate prediction heads to predict all key 3D attributes.

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=1.0\linewidth, height=6cm]{sec/figures/sim.pdf}
  \caption{The figure shows the attention between a randomly selected token from Image10 (as the query) and all other tokens (as values) from three images. The color represents the attention weight, with darker colors indicating higher attention. Each row corresponds to different layers, and each column shows attention patterns across images, demonstrating high similarity between tokens across frames. The similarity of attention maps across adjacent layers indicates the stability of token similarity between layers.}
  \label{fig:sim}
\end{figure*}


\subsection{Speed Bottleneck Analysis}
VGGT employs a two-stage attention mechanism: Frame Attention captures intra-frame details, focusing on local variations, while Global Attention models inter-frame dependencies to ensure global consistency. However, maintaining this consistency requires concatenating tokens from all input images and performing self-attention across the entire sequence, resulting in quadratic complexity. As the number of input images increases, the computational cost of Global Attention grows rapidly, becoming a significant speed bottleneck when scaling to larger scenes. This limitation is clearly highlighted in Figure \ref{fig:global_time}.

We hypothesize that Global Attention in scene reconstruction suffers from redundancy and inefficiency. Since DinoV2 extracts local semantic information, many images in a scene share overlapping regions with the same semantic content, leading to unnecessary computation. As shown in Figure \ref{fig:sim}, we visualize VGGT’s Global Attention maps on the "Barn" scene from the Tanks and Temples dataset. We randomly sampled a token and visualized its attention map across four images. The token consistently maintains high attention across frames, focusing on the same semantic region (e.g., the roof), which demonstrates high similarity between tokens across frames. This observation validates our hypothesis and motivates the introduction of our gs-driven and cached token merging strategy.


\subsection{eometry-aware and Cached Token Merging}
As shown in Fig \ref{fig:pipeline}, our proposed gs-driven and cached token merging strategy consists of four stages: gs-driven token partitioning, token merging and unmerging, and caching of merging indices.

% Cross-Frame Geometric Correspondence
% Without considering these cross-frame correspondences, important geometric information is often lost during token merging.
%  where information relevant to the 3D structure is not preserved adequately.


\textbf{Token partition.} Conventional Traditional token merging strategies typically partition tokens into destination (dst) and source (src) sets through random or fixed-stride sampling. However, this approach fails to account for the complex geometric relationships in 3D scenes, leading to suboptimal performance in 3D reconstruction tasks.

Specifically, two key issues arise:
(1) Randomly selecting tokens as dst or src can lead to the merging of high-information tokens, such as object edges or textured surfaces, with low-information tokens. This results in the loss of critical geometric features, which are essential for precise cross-frame matching and accurate 3D reconstruction.
(2) The random selection of dst tokens often fails to identify smooth surfaces (e.g., walls, sky), which are more suitable for efficient merging. Additionally, a high merge ratio risks merging high-information tokens, which reduces merge efficiency and degrades reconstruction quality.
Thus, it is essential to design an efficient token partitioning strategy that facilitates better cross-frame merging without increasing complexity.

In 3D reconstruction feed-forward models, preserving critical texture and geometric details is crucial for accurate spatial information. Therefore, we design a token merging classification tailored for 3D reconstruction, categorizing tokens into src, dst, and salient, ensuring that salient tokens are not involved in merging.We then use the newly introduced info map concept to guide the classification of src, dst, and salient tokens.

%  通过我们的策略，token能够保留更完整的信息，捕捉到更细致的纹理复杂度和几何结构，为后续的重建提供更精确的空间信息。

%  选择性地保留具有更高信息量的token，特别是边缘等关键区域，有助于在多视角重建中保持一致性，提高跨帧匹配的精度，最终优化3D重建质量。

\begin{figure*}[htbp]
\centering
\includegraphics[width=1\linewidth]{sec/figures/GA_map.pdf}
\caption{The visualizations of pixel gradients (Grid map) and token variance (Variance map). The Geometry-aware(GA) map represents the weighted sum of these two maps, highlighting regions with high information content (typically corresponding to areas with rich semantic information or textures) and dimming regions with lower information content.}
\label{fig:info_map}
\end{figure*}


\textbf{Feature map.} 
Naturally, tokens representing object edges or textured regions are protected to preserve detail, while large empty areas, like the sky or walls, are selected as dst tokens to lead the merging process. This aligns with common sense, minimizing redundant computations and preserving essential geometric features.
Building on this insight, we introduce the info map, which quantifies the geometric and semantic information of each token. 
To achieve this, we define two key components of the info map: \textbf{pixel gradients} and \textbf{token variances}. 

The pixel gradient captures the geometric detail of each token, quantifying the intensity of spatial changes in the image, such as edges and textures.
We firstly converted all input images to grayscale to simplify the gradient computation. 
The gradient of an image \( I(x, y) \) represents the rate of change of intensity at each pixel, measured in both the horizontal (\(G_x\)) and vertical (\(G_y\)) directions. These gradients are approximated using the Sobel operator, which computes the discrete partial derivatives of the image.

Let \( (x, y) \) denote the pixel coordinates in the image, and \( I(x, y) \) represents the intensity of the image at that point. The gradients in the horizontal and vertical directions can be approximated as follows:


These kernels are convolved with the image to approximate the gradients \( G_x \) and \( G_y \), which represent the intensity changes along the horizontal and vertical directions, respectively.

To obtain the gradient magnitude \( G \) at each pixel, the horizontal and vertical gradients are combined as follows:

\[
G = \sqrt{G_x^2 + G_y^2}
\]

The gradient magnitude \( G \) indicates the overall rate of intensity change at each pixel, where higher values correspond to stronger changes, such as those found at edges in the image.
Finally, all pixel gradient information are downsampled to the token grid, as the \text{grid\_map}.

The token variance measure the variability of semantic information within a token's region. By calculating the variance between a token and its surrounding tokens, we quantify the degree of semantic change in the corresponding image region.
To calculate token variances, we first rearrange the tokens into a 2D grid of image patches. Then, we apply two rounds of average pooling with a \(3 \times 3\) window to compute the local mean and squared mean. Finally, we compute the variance by subtracting the squared mean from the mean of the squared values:
\[
\text{var\_map} = \text{avg\_pool}(X^2) - (\text{avg\_pool}(X))^2
\]
where \( X \) represents the projected token features. This variance map reflects the variability of semantic features, helping to identify regions with more dynamic or complex information.

The pixel gradient map (\(\text{grid\_map}\)) and the token variance map (\(\text{var\_map}\)) are first normalized then combined to form the final info map:
\[
\text{info\_map} = \alpha \cdot \text{norm}(\text{grid\_map}) + \beta \cdot \text{norm}(\text{var\_map})
\]
The resulting token-wise info map integrates both the geometric and semantic information, providing a comprehensive representation for each patch token. 
Both the Sobel operator and average pooling are highly efficient operations, introducing almost no latency in the computation.
As shown in Figure \ref{fig:info_map}, the highlighted tokens in the info map represent texture-rich areas with high information content, which are crucial for precise cross-frame matching and accurate 3D reconstruction. In contrast, the dimmed tokens indicate smooth regions with low variance, which are better suited as dst tokens for the merging process.

\textbf{Salient token selection.} 
We select the top 10\% highest-information tokens in each image as salient tokens, which are excluded from the merge process. By selectively retaining these tokens, particularly those in key regions like edges, we preserve the most important details of the scene. This helps maintain consistency in multi-view reconstruction, improves cross-frame matching accuracy, and ultimately enhances the quality of the 3D reconstruction.

\textbf{Dst token sample strategy.}
VGGT defines the first frame as the world coordinate system, which makes all tokens from the first frame highly representative and crucial for maintaining spatial coherence. Therefore, we designate all tokens from the first frame as dst tokens.
For other frames, we adopt a strategy inspired by ToMe, where we first partition the input tokens by frame and arrange them into a 2D grid of image patches. Then, one token is selected per 2×2 patch to serve as the dst token. This region-based strategy ensures spatially balanced merging and prevents artifacts such as the disappearance of large areas.
Specifically, We choose the lowest information token within each patch as the dst token, ensuring that smoother, less complex regions are selected. This increases merging efficiency, as regions like large areas of sky with dst tokens can be merged quickly, while more detailed tokens are excluded from merging.




\textbf{Token merging.}
Tokens not selected as dst or salient tokens are assigned as src tokens. Src tokens are then merged into their most similar counterparts in dst tokens, effectively reducing the sequence length for global attention computation. Formally, given a token representation \( x \in \mathbb{R}^c \) with feature dimension \( c \), we compute the cosine similarity between each src token \( x_s \) and all dst tokens \( x_d \in \text{dst} \):

\[
\text{sim}(x_s, x_d) = \frac{x_s \cdot x_d}{\|x_s\| \|x_d\|}
\]

Each src token \( x_s \) is assigned to its most similar dst token \( x_d \), and updated by averaging:

\[
x_s' = \frac{x_d + x_s}{2}
\]

The updated \( x_s' \) is retained while \( x_s \) is temporarily discarded, thereby reducing the number of tokens processed in attention computations.


\textbf{Token unmerging.}
This module is essential for VGGT, as it restores tokens to their original shape for dense prediction output.
Specifically, two tokens \( x_1, x_2 \in \mathbb{R}^c \) are merged into a single representation:

\[
x_{1,2}^* = \frac{x_1 + x_2}{2}
\]

During unmerging, the representation is replicated to restore the original token shape:

\[
x_1' = x_{1,2}^*, \quad x_2' = x_{1,2}^*
\]

The two replicated tokens can then regain their distinctiveness through Frame Attention, which reintroduces local variability.



\textbf{Caching merging indices.} Introducing the token merge module into the 24-layer Global Attention significantly accelerated processing. However, as shown in Figure \ref{fig:CM}, computing merging indices at each layer incurs a notable time overhead. We questioned whether it was necessary to compute merging indices at every layer?
Based on the token similarity observed in Figure \ref{fig:sim}, we found that token similarity remains stable between adjacent layers, as the regions attended by tokens are almost identical across these layers. This insight led us to cache and reuse previously computed merging indices. By limiting merge index computation to just four layers, we achieved a 20\% reduction in latency while maintaining accuracy.


\begin{figure}[htbp]
\centering
\includegraphics[width=0.7\linewidth,height=4cm]{sec/figures/CM.pdf}
\caption{Latency analysis of the VGGT components after introducing token merge. CM refers to the latency of calculating the merge indices. As image input increases, CM also becomes a speed bottleneck.}
\label{fig:CM}
\end{figure}


\subsection{Fine-tuning and FP8 Quantization}
We employ fine-tuning and FP8 quantization to maximize the acceleration of VGGT while carefully managing the trade-off with accuracy.

\textbf{fine-tuning.} To further preserve our LiteVGGT's accuracy and performance after introducing the merge module, we fine-tune both the aggregator and the prediction heads based on VGGT's pretrained checkpoints. We use a diverse mixture of synthetic and real-world datasets, including Co3Dv2, BlendMVS, DL3DV, MegaDepth, WildRGB, ScanNet++, HyperSim, Mapillary, Replica, MVS-Synth, and Virtual KITTI. For each batch, we sample 4–48 images. The model is trained for 20K iterations on 8 H20 GPUs, taking approximately three days.
 
\textbf{FP8 quantization.} This reduces model memory footprint and computational cost by lowering precision to 8 bits. We carefully switch our model to FP8 inference using NVIDIA's \textit{transformer engine} library after weight mapping, achieving a significant reduction in both latency and memory usage, with minimal impact on performance.



